ModalPINN: an extension of Physics-Informed Neural Networks with enforced truncated Fourier decomposition for periodic flow reconstruction using a limited number of imperfect sensors

Continuous reconstructions of periodic phenomena provide powerful tools to understand, predict and model natural situations and engineering problems. In line with the recent method called Physics-Informed Neural Networks (PINN) where a multi layer perceptron directly approximates any physical quantity as a symbolic function of time and space coordinates, we present an extension, namely ModalPINN, that encodes the approximation of a limited number of Fourier mode shapes. In addition to the added interpretability, this representation performs up to two orders of magnitude more precisely for a similar number of degrees of freedom and training time in some cases as illustrated through the test case of laminar shedding of vortices over a cylinder. This added simplicity proves to be robust in regards to flow reconstruction using only a limited number of sensors with asymmetric data that simulates an experimental configuration, even when a Gaussian noise or a random delay is added, imitating imperfect and sparse information.

==> Python_data_figure/FBC5/Coupe_FBC5.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\begin{axis}[
width = 11.1cm,
height=3cm,
tick align=outside,
tick pos=left,
xmin=-4, xmax=8,
axis x line = none,
axis y line = left,
y grid style={white!69.0196078431373!black},
ymin=-0.1, ymax=1.2,
ytick style={color=black},
ytick={0,1},
yticklabels={\(\displaystyle 0\),\(\displaystyle 1\)}
]
\addplot [semithick, black]
table {%
-4 0.999999999999999
-3.87878787878788 0.999999999999996
-3.75757575757576 0.999999999999986
-3.63636363636364 0.999999999999952
-3.51515151515152 0.999999999999839
-3.39393939393939 0.999999999999459
-3.27272727272727 0.999999999998184
-3.15151515151515 0.999999999993896
-3.03030303030303 0.999999999979485
-2.90909090909091 0.999999999931058
-2.78787878787879 0.999999999768315
-2.66666666666667 0.999999999221397
-2.54545454545455 0.999999997383421
-2.42424242424242 0.999999991206711
-2.3030303030303 0.999999970449225
-2.18181818181818 0.999999900691502
-2.06060606060606 0.999999666263338
-1.93939393939394 0.999998878443129
-1.81818181818182 0.999996230894625
-1.6969696969697 0.999987333579513
-1.57575757575758 0.999957433792061
-1.45454545454545 0.999856958947428
-1.33333333333333 0.999519376574362
-1.21212121212121 0.998385729943032
-1.09090909090909 0.994585391520763
-0.96969696969697 0.981919188382134
-0.848484848484849 0.940507149231852
-0.727272727272727 0.813185990566335
-0.606060606060606 0.485612694471235
-0.484848484848485 0
-0.363636363636363 0
-0.242424242424242 0
-0.121212121212121 0
0 0
0.121212121212121 0
0.242424242424242 0
0.363636363636363 0
0.484848484848485 0
0.606060606060606 0.485612694471237
0.727272727272728 0.813185990566336
0.848484848484849 0.940507149231852
0.96969696969697 0.981919188382134
1.09090909090909 0.994585391520763
1.21212121212121 0.998385729943032
1.33333333333333 0.999519376574362
1.45454545454546 0.999856958947428
1.57575757575758 0.999957433792061
1.6969696969697 0.999987333579513
1.81818181818182 0.999996230894625
1.93939393939394 0.999998878443129
2.06060606060606 0.999999666263338
2.18181818181818 0.999999900691502
2.3030303030303 0.999999970449225
2.42424242424242 0.999999991206711
2.54545454545455 0.999999997383421
2.66666666666667 0.999999999221397
2.78787878787879 0.999999999768315
2.90909090909091 0.999999999931058
3.03030303030303 0.999999999979485
3.15151515151515 0.999999999993896
3.27272727272727 0.999999999998184
3.39393939393939 0.999999999999459
3.51515151515152 0.999999999999839
3.63636363636364 0.999999999999952
3.75757575757576 0.999999999999986
3.87878787878788 0.999999999999996
4 0.999999999999999
4.12121212121212 1
4.24242424242424 1
4.36363636363636 1
4.48484848484848 1
4.60606060606061 1
4.72727272727273 1
4.84848484848485 1
4.96969696969697 1
5.09090909090909 1
5.21212121212121 1
5.33333333333333 1
5.45454545454546 1
5.57575757575758 1
5.6969696969697 1
5.81818181818182 1
5.93939393939394 1
6.06060606060606 1
6.18181818181818 1
6.3030303030303 1
6.42424242424242 1
6.54545454545454 1
6.66666666666667 1
6.78787878787879 1
6.90909090909091 1
7.03030303030303 1
7.15151515151515 1
7.27272727272727 1
7.39393939393939 1
7.51515151515152 1
7.63636363636364 1
7.75757575757576 1
7.87878787878788 1
8 1
};
\addplot [semithick, black, dashed]
table {%
-4 -0
-3.87878787878788 -0
-3.75757575757576 -0
-3.63636363636364 -0
-3.51515151515152 -0
-3.39393939393939 -0
-3.27272727272727 -0
-3.15151515151515 -0
-3.03030303030303 -0
-2.90909090909091 -0
-2.78787878787879 -0
-2.66666666666667 -0
-2.54545454545455 -0
-2.42424242424242 -0
-2.3030303030303 -0
-2.18181818181818 -0
-2.06060606060606 -0
-1.93939393939394 -0
-1.81818181818182 -0
-1.6969696969697 -0
-1.57575757575758 -0
-1.45454545454545 -0
-1.33333333333333 -0
-1.21212121212121 -0
-1.09090909090909 -0
-0.96969696969697 -0
-0.848484848484849 -0
-0.727272727272727 -0
-0.606060606060606 -0
-0.484848484848485 -0
-0.363636363636363 -0
-0.242424242424242 -0
-0.121212121212121 -0
0 0
0.121212121212121 0
0.242424242424242 0
0.363636363636363 0
0.484848484848485 0
0.606060606060606 0
0.727272727272728 0
0.848484848484849 0
0.96969696969697 0
1.09090909090909 0
1.21212121212121 0
1.33333333333333 0
1.45454545454546 0
1.57575757575758 0
1.6969696969697 0
1.81818181818182 0
1.93939393939394 0
2.06060606060606 0
2.18181818181818 0
2.3030303030303 0
2.42424242424242 0
2.54545454545455 0
2.66666666666667 0
2.78787878787879 0
2.90909090909091 0
3.03030303030303 0
3.15151515151515 0
3.27272727272727 0
3.39393939393939 0
3.51515151515152 0
3.63636363636364 0
3.75757575757576 0
3.87878787878788 0
4 0
4.12121212121212 0
4.24242424242424 0
4.36363636363636 0
4.48484848484848 0
4.60606060606061 0
4.72727272727273 0
4.84848484848485 0
4.96969696969697 0
5.09090909090909 0
5.21212121212121 0
5.33333333333333 0
5.45454545454546 0
5.57575757575758 0
5.6969696969697 0
5.81818181818182 0
5.93939393939394 0
6.06060606060606 0
6.18181818181818 0
6.3030303030303 0
6.42424242424242 0
6.54545454545454 0
6.66666666666667 0
6.78787878787879 0
6.90909090909091 0
7.03030303030303 0
7.15151515151515 0
7.27272727272727 0
7.39393939393939 0
7.51515151515152 0
7.63636363636364 0
7.75757575757576 0
7.87878787878788 0
8 0
};
\end{axis}

\end{tikzpicture}


==> Python_data_figure/Mes_point_result/ModalPINN_VS_ExpMes_2020_10_29-09_26_24__357/Forces.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Time \(\displaystyle t\)},
xmin=399.0885955, xmax=420.9032345,
xtick style={color=black},
xtick={395,400,405,410,415,420,425},
xticklabels={\(\displaystyle 395\),\(\displaystyle 400\),\(\displaystyle 405\),\(\displaystyle 410\),\(\displaystyle 415\),\(\displaystyle 420\),\(\displaystyle 425\)},
y grid style={white!69.0196078431373!black},
ylabel={Forces},
ymin=-0.203642007703835, ymax=0.711679821780525,
ytick style={color=black},
ytick={-0.4,-0.2,0,0.2,0.4,0.6,0.8},
yticklabels={\(\displaystyle -0.4\),\(\displaystyle -0.2\),\(\displaystyle 0.0\),\(\displaystyle 0.2\),\(\displaystyle 0.4\),\(\displaystyle 0.6\),\(\displaystyle 0.8\)}
]
\addplot [semithick, color0]
table {%
400.08017 0.66265895
400.19165 0.66180014
400.30305 0.66110401
400.41439 0.66060713
400.52567 0.6603356
400.63684 0.66030324
400.74793 0.66051093
400.85907 0.66094756
400.97021 0.66158977
401.08125 0.66240257
401.19224 0.6633431
401.30333 0.66436308
401.4145 0.66540879
401.52564 0.66642421
401.63678 0.66735637
401.74805 0.66815725
401.85943 0.6687841
401.97082 0.66920296
402.08224 0.66939164
402.19376 0.66933968
402.30533 0.66904914
402.41691 0.66853507
402.52852 0.6678243
402.64015 0.66695439
402.75178 0.66597163
402.86341 0.66492834
402.97502 0.66388043
403.08661 0.66288389
403.1982 0.66199192
403.30973 0.66125251
403.4212 0.66070502
403.53267 0.66037805
403.64419 0.66028896
403.75567 0.66044236
403.86706 0.66082936
403.97844 0.66142915
404.08985 0.66220981
404.20121 0.66312934
404.31252 0.66413878
404.42384 0.66518519
404.53521 0.66621379
404.64665 0.66717047
404.75815 0.66800445
404.86965 0.66867128
404.98116 0.66913569
405.09274 0.66937308
405.20442 0.66937022
405.31612 0.66912668
405.42777 0.66865532
405.53941 0.66798102
405.65108 0.66713912
405.76277 0.66617431
405.8744 0.66513859
405.98597 0.66408754
406.09751 0.66307684
406.20902 0.66216049
406.32045 0.6613877
406.43182 0.66079929
406.54313 0.66042613
406.65435 0.66028768
406.76546 0.66039042
406.87657 0.66072845
406.98773 0.66128389
407.09882 0.66202655
407.20981 0.66291651
407.32085 0.66390784
407.432 0.66494912
407.54316 0.66598468
407.65428 0.66695967
407.76548 0.66782392
407.87683 0.66853216
407.98822 0.66904599
408.09961 0.66933791
408.21109 0.66939236
408.32265 0.66920568
408.43423 0.66878732
408.54582 0.66815908
408.65745 0.66735394
408.76907 0.66641468
408.8807 0.66539128
408.99232 0.66433842
409.10392 0.6633125
409.21551 0.66236824
409.32708 0.66155626
409.43857 0.66092015
409.55003 0.66049333
409.66153 0.6602982
409.77304 0.66034522
409.88447 0.66063135
409.99584 0.66114079
410.10724 0.6618465
410.21863 0.66271064
410.32996 0.66368685
410.44127 0.66472369
410.55261 0.6657669
410.66402 0.66676174
410.7755 0.66765564
410.887 0.66840096
410.9985 0.66895811
411.11004 0.66929772
411.22169 0.66940141
411.33339 0.66926296
411.44506 0.66888945
411.5567 0.66830068
411.66835 0.66752754
411.78004 0.66661077
411.89171 0.66559952
412.0033 0.66454831
412.11484 0.66351306
412.22637 0.66254876
412.33784 0.66170721
412.44923 0.66103326
412.56057 0.66056228
412.67185 0.66031898
412.783 0.66031563
412.89409 0.66055161
413.00524 0.66101439
413.11637 0.66167912
413.22739 0.66250962
413.33839 0.66346235
413.44949 0.66448834
413.56067 0.66553337
413.6718 0.66654149
413.78295 0.66746034
413.89424 0.66824246
414.00562 0.66884592
414.11701 0.6692381
414.22844 0.66939821
414.33997 0.66931726
414.45155 0.66899884
414.56313 0.66845954
414.67474 0.66772749
414.78637 0.66684145
414.898 0.66584857
415.00963 0.66480173
415.12123 0.66375706
415.23282 0.66277033
415.34441 0.66189428
415.45594 0.66117602
415.5674 0.6606537
415.67888 0.6603546
415.7904 0.66029462
415.90187 0.66047678
416.01325 0.66089064
416.12464 0.66151403
416.23604 0.66231375
416.34739 0.66324676
416.4587 0.66426348
416.57003 0.66531066
416.68141 0.66633344
416.79286 0.66727798
416.90435 0.66809409
417.01585 0.66873829
417.12737 0.66917654
417.23896 0.66938555
417.35065 0.66935357
417.46234 0.66908175
417.574 0.6685845
417.68563 0.66788803
417.79731 0.66702885
417.90899 0.66605267
418.02062 0.66501215
418.13218 0.66396302
418.24372 0.66296085
418.35522 0.66205927
418.46664 0.66130663
418.578 0.66074263
418.68931 0.66039686
418.80052 0.66028727
418.91162 0.66041879
419.02274 0.6607841
419.13389 0.66136384
419.24497 0.66212642
419.35595 0.66303107
419.467 0.66403122
419.57816 0.6650748
419.68932 0.66610591
419.80044 0.66707016
419.91166 0.66791798
};
\addplot [semithick, color1, dashed]
table {%
400.08017 0.66237884759903
400.19165 0.661387979984283
400.30305 0.660601615905762
400.41439 0.66006600856781
400.52567 0.659810185432434
400.63684 0.65984582901001
400.74793 0.660166203975677
400.85907 0.660749018192291
400.97021 0.661557018756866
401.08125 0.662539958953857
401.19224 0.663641691207886
401.30333 0.664802730083466
401.4145 0.665960431098938
401.52564 0.667055904865265
401.63678 0.66803640127182
401.74805 0.668858051300049
401.85943 0.669485569000244
401.97082 0.669893324375153
402.08224 0.670068442821503
402.19376 0.670007824897766
402.30533 0.669718384742737
402.41691 0.669216632843018
402.52852 0.668526172637939
402.64015 0.667678475379944
402.75178 0.666710376739502
402.86341 0.665662169456482
402.97502 0.664578914642334
403.08661 0.663506865501404
403.1982 0.662492275238037
403.30973 0.661582291126251
403.4212 0.660819292068481
403.53267 0.660241067409515
403.64419 0.659879446029663
403.75567 0.659757137298584
403.86706 0.659885942935944
403.97844 0.660265207290649
404.08985 0.660881161689758
404.20121 0.661706209182739
404.31252 0.662700295448303
404.42384 0.663811206817627
404.53521 0.664979636669159
404.64665 0.666138768196106
404.75815 0.667220234870911
404.86965 0.668157756328583
404.98116 0.668891787528992
405.09274 0.669375479221344
405.20442 0.669575214385986
405.31612 0.669475078582764
405.42777 0.669079184532166
405.53941 0.668410181999207
405.65108 0.667508363723755
405.76277 0.666430950164795
405.8744 0.66524475812912
405.98597 0.66402542591095
406.09751 0.662849068641663
406.20902 0.661788165569305
406.32045 0.660908222198486
406.43182 0.66026109457016
406.54313 0.659883737564087
406.65435 0.659794986248016
406.76546 0.659995973110199
406.87657 0.66047066450119
406.98773 0.661188244819641
407.09882 0.662103235721588
407.20981 0.66316169500351
407.32085 0.664304912090302
407.432 0.665471851825714
407.54316 0.666600704193115
407.65428 0.667635858058929
407.76548 0.66852992773056
407.87683 0.66924387216568
407.98822 0.669747591018677
408.09961 0.670022666454315
408.21109 0.670062124729156
408.32265 0.66986882686615
408.43423 0.66945481300354
408.54582 0.66884171962738
408.65745 0.668056786060333
408.76907 0.667134881019592
408.8807 0.666115701198578
408.99232 0.66504180431366
409.10392 0.663959145545959
409.21551 0.662914574146271
409.32708 0.661954402923584
409.43857 0.661123752593994
409.55003 0.660462617874146
409.66153 0.660005390644073
409.77304 0.659779012203217
409.88447 0.659800231456757
409.99584 0.660073459148407
410.10724 0.660591125488281
410.21863 0.661331653594971
410.32996 0.662259221076965
410.44127 0.663327395915985
410.55261 0.664479196071625
410.66402 0.66565066576004
410.7755 0.666773796081543
410.887 0.667779803276062
410.9985 0.668607234954834
411.11004 0.669202506542206
411.22169 0.669526278972626
411.33339 0.669554531574249
411.44506 0.669282913208008
411.5567 0.66872626543045
411.66835 0.667917966842651
411.78004 0.66690731048584
411.89171 0.66575825214386
412.0033 0.664543986320496
412.11484 0.663340032100677
412.22637 0.662221491336823
412.33784 0.661257266998291
412.44923 0.660505771636963
412.56057 0.660009980201721
412.67185 0.659797072410583
412.783 0.659875690937042
412.89409 0.660236835479736
413.00524 0.660855710506439
413.11637 0.66169285774231
413.22739 0.66269713640213
413.33839 0.663811326026917
413.44949 0.664975702762604
413.56067 0.666128098964691
413.6718 0.667209684848785
413.78295 0.66816908121109
413.89424 0.668963968753815
414.00562 0.669560074806213
414.11701 0.669934034347534
414.22844 0.670074284076691
414.33997 0.669979214668274
414.45155 0.669657111167908
414.56313 0.669125497341156
414.67474 0.668410003185272
414.78637 0.667541921138763
414.898 0.666558861732483
415.00963 0.665502846240997
415.12123 0.664418518543243
415.23282 0.663351774215698
415.34441 0.662350058555603
415.45594 0.661459147930145
415.5674 0.660721302032471
415.67888 0.660173296928406
415.7904 0.659845769405365
415.90187 0.659760355949402
416.01325 0.659926414489746
416.12464 0.66034197807312
416.23604 0.660990953445435
416.34739 0.66184401512146
416.4587 0.662858724594116
416.57003 0.663982272148132
416.68141 0.665153503417969
416.79286 0.666305422782898
416.90435 0.667369782924652
417.01585 0.668280124664307
417.12737 0.668980240821838
417.23896 0.669423460960388
417.35065 0.669579386711121
417.46234 0.66943484544754
417.574 0.668996453285217
417.68563 0.668290257453918
417.79731 0.667358756065369
417.90899 0.666260063648224
418.02062 0.665064454078674
418.13218 0.663846790790558
418.24372 0.662682831287384
418.35522 0.6616450548172
418.46664 0.660796582698822
418.578 0.660187602043152
418.68931 0.659852147102356
418.80052 0.659806728363037
418.91162 0.660049557685852
419.02274 0.660562694072723
419.13389 0.661312639713287
419.24497 0.66225266456604
419.35595 0.663327395915985
419.467 0.66447788476944
419.57816 0.665642559528351
419.68932 0.666761338710785
419.80044 0.667778313159943
419.91166 0.668647825717926
};
\addplot [semithick, color2, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
400.08017 0.019452365
400.19165 0.00082595482
400.30305 -0.017823055
400.41439 -0.036252194
400.52567 -0.054212695
400.63684 -0.07145315
400.74793 -0.087747648
400.85907 -0.10288897
400.97021 -0.11666154
401.08125 -0.12886365
401.19224 -0.13933821
401.30333 -0.14795541
401.4145 -0.1545944
401.52564 -0.15916143
401.63678 -0.1616036
401.74805 -0.16189495
401.85943 -0.16003304
401.97082 -0.15605006
402.08224 -0.1500052
402.19376 -0.14197773
402.30533 -0.13207828
402.41691 -0.12044238
402.52852 -0.10721965
402.64015 -0.092582119
402.75178 -0.076720103
402.86341 -0.059836271
402.97502 -0.042150431
403.08661 -0.023890474
403.1982 -0.0052916919
403.30973 0.013394412
403.4212 0.031916296
403.53267 0.050037844
403.64419 0.067519465
403.75567 0.0841073
403.86706 0.099566848
403.97844 0.11369648
404.08985 0.12630308
404.20121 0.137206
404.31252 0.14625769
404.42384 0.15334185
404.53521 0.15836743
404.64665 0.16126968
404.75815 0.16201283
404.86965 0.16059349
404.98116 0.15703911
405.09274 0.15140107
405.20442 0.14375595
405.31612 0.13421243
405.42777 0.12290535
405.53941 0.10998327
405.65108 0.095608396
405.76277 0.079966299
405.8744 0.06326761
405.98597 0.045731335
406.09751 0.027576533
406.20902 0.0090389852
406.32045 -0.0096302792
406.43182 -0.028186056
406.54313 -0.046384181
406.65435 -0.063971299
406.76546 -0.080707845
406.87657 -0.096382432
406.98773 -0.11078404
407.09882 -0.12369926
407.20981 -0.13495076
407.32085 -0.14440068
407.432 -0.1519239
407.54316 -0.15741141
407.65428 -0.1607929
407.76548 -0.16203258
407.87683 -0.1611163
407.98822 -0.15806048
408.09961 -0.15291444
408.21109 -0.14574775
408.32265 -0.13665628
408.43423 -0.12576688
408.54582 -0.11322267
408.65745 -0.099184956
408.76907 -0.083837596
408.8807 -0.067377282
408.99232 -0.050016414
409.10392 -0.031980823
409.21551 -0.013501073
409.32708 0.0051782451
409.43857 0.02380233
409.55003 0.042128615
409.66153 0.059922605
409.77304 0.076934714
409.88447 0.092917049
409.99584 0.10765567
410.10724 0.12095599
410.21863 0.13262888
410.32996 0.14251104
410.44127 0.15047359
410.55261 0.15641452
410.66402 0.16025722
410.7755 0.16195275
410.887 0.16148319
410.9985 0.15886317
411.11004 0.15413418
411.22169 0.14736073
411.33339 0.13863711
411.44506 0.12808831
411.5567 0.11585782
411.66835 0.10210092
411.78004 0.086991725
411.89171 0.070730936
412.0033 0.053536419
412.11484 0.035626131
412.22637 0.017226451
412.33784 -0.0014157133
412.44923 -0.020051091
412.56057 -0.038437383
412.67185 -0.056324484
412.783 -0.073462687
412.89409 -0.089629758
413.00524 -0.10461836
413.11637 -0.11821234
413.22739 -0.13021457
413.33839 -0.1404729
413.44949 -0.14885881
413.56067 -0.15525328
413.6718 -0.1595674
413.78295 -0.16175245
413.89424 -0.16178491
414.00562 -0.15966605
414.11701 -0.15543215
414.22844 -0.14914467
414.33997 -0.14088604
414.45155 -0.13077075
414.56313 -0.11893617
414.67474 -0.10553408
414.78637 -0.090739337
414.898 -0.074743672
415.00963 -0.05775169
415.12123 -0.039984874
415.23282 -0.021671532
415.34441 -0.0030487316
415.45594 0.015630664
415.5674 0.034116752
415.67888 0.052174529
415.7904 0.069562324
415.90187 0.086026368
416.01325 0.10133657
416.12464 0.1152936
416.23604 0.12770475
416.34739 0.13839259
416.4587 0.14721378
416.57003 0.15405521
416.68141 0.15882884
416.79286 0.16147326
416.90435 0.1619564
417.01585 0.16027886
417.12737 0.15647128
417.23896 0.15058773
417.35065 0.14270841
417.46234 0.13294577
417.574 0.12143682
417.68563 0.10833146
417.79731 0.093794154
417.90899 0.078013759
418.02062 0.061203035
418.13218 0.043580823
418.24372 0.025367159
418.35522 0.0068005066
418.46664 -0.011867886
418.578 -0.030393829
418.68931 -0.048532063
418.80052 -0.066029138
418.91162 -0.082649052
419.02274 -0.098182302
419.13389 -0.11241644
419.24497 -0.12514037
419.35595 -0.13618249
419.467 -0.14540768
419.57816 -0.15269174
419.68932 -0.15792937
419.80044 -0.16105524
419.91166 -0.16203647
};
\addplot [semithick, color3, dotted]
table {%
400.08017 0.0192217398434877
400.19165 0.000733421358745545
400.30305 -0.0177910476922989
400.41439 -0.0361077040433884
400.52567 -0.0539669916033745
400.63684 -0.0711316093802452
400.74793 -0.0873579829931259
400.85907 -0.102446883916855
400.97021 -0.116178400814533
401.08125 -0.128348365426064
401.19224 -0.138800755143166
401.30333 -0.147404164075851
401.4145 -0.154032900929451
401.52564 -0.158598840236664
401.63678 -0.161047026515007
401.74805 -0.161351889371872
401.85943 -0.159510746598244
401.97082 -0.155556231737137
402.08224 -0.149544298648834
402.19376 -0.141556516289711
402.30533 -0.131694868206978
402.41691 -0.120097525417805
402.52852 -0.106900110840797
402.64015 -0.092282846570015
402.75178 -0.0764273554086685
402.86341 -0.0595296658575535
402.97502 -0.0418144091963768
403.08661 -0.0235109888017178
403.1982 -0.00484979571774602
403.30973 0.013900519348681
403.4212 0.032490573823452
403.53267 0.0506789460778236
403.64419 0.0682064592838287
403.75567 0.0848254263401031
403.86706 0.100283809006214
403.97844 0.114383704960346
404.08985 0.126918748021126
404.20121 0.137715816497803
404.31252 0.146631926298141
404.42384 0.153547704219818
404.53521 0.158386617898941
404.64665 0.16109074652195
404.75815 0.161635249853134
404.86965 0.160026863217354
404.98116 0.15630441904068
405.09274 0.150526896119118
405.20442 0.142778232693672
405.31612 0.13316747546196
405.42777 0.121841661632061
405.53941 0.108936101198196
405.65108 0.0946100652217865
405.76277 0.0790582448244095
405.8744 0.0624667666852474
405.98597 0.0450515598058701
406.09751 0.0270316861569881
406.20902 0.00862634088844061
406.32045 -0.00991310738027096
406.43182 -0.028348920866847
406.54313 -0.0464315041899681
406.65435 -0.0639219060540199
406.76546 -0.0805728808045387
406.87657 -0.09616868942976
406.98773 -0.110507115721703
407.09882 -0.123364984989166
407.20981 -0.134566724300385
407.32085 -0.143973469734192
407.432 -0.151458486914635
407.54316 -0.156911179423332
407.65428 -0.160265192389488
407.76548 -0.161484867334366
407.87683 -0.160556331276894
407.98822 -0.157495707273483
408.09961 -0.15235324203968
408.21109 -0.145194172859192
408.32265 -0.136115819215775
408.43423 -0.125238731503487
408.54582 -0.112709522247314
408.65745 -0.0986734852194786
408.76907 -0.0833177417516708
408.8807 -0.0668409243226051
408.99232 -0.0494486205279827
409.10392 -0.0313642360270023
409.21551 -0.0128283072263002
409.32708 0.00591850094497204
409.43857 0.0246087778359652
409.55003 0.0429920107126236
409.66153 0.0608366020023823
409.77304 0.0778722763061523
409.88447 0.0938538536429405
409.99584 0.108556002378464
410.10724 0.121779106557369
410.21863 0.133340820670128
410.32996 0.143071472644806
410.44127 0.150851666927338
410.55261 0.156584411859512
410.66402 0.160202354192734
410.7755 0.161667734384537
410.887 0.1609738022089
410.9985 0.158145099878311
411.11004 0.153235107660294
411.22169 0.14631399512291
411.33339 0.137479901313782
411.44506 0.126866027712822
411.5567 0.114616088569164
411.66835 0.100878529250622
411.78004 0.0858214423060417
411.89171 0.0696439445018768
412.0033 0.0525572001934052
412.11484 0.0347667410969734
412.22637 0.0164970997720957
412.33784 -0.00201328401453793
412.44923 -0.0205189827829599
412.56057 -0.0387855358421803
412.67185 -0.0565630979835987
412.783 -0.0735969468951225
412.89409 -0.0896718502044678
413.00524 -0.104572497308254
413.11637 -0.118082582950592
413.22739 -0.130008637905121
413.33839 -0.140194281935692
413.44949 -0.148511812090874
413.56067 -0.154841423034668
413.6718 -0.159096255898476
413.78295 -0.161227732896805
413.89424 -0.161214202642441
414.00562 -0.159057915210724
414.11701 -0.154795289039612
414.22844 -0.148484200239182
414.33997 -0.140213012695312
414.45155 -0.130085527896881
414.56313 -0.118236638605595
414.67474 -0.1048244535923
414.78637 -0.0900080651044846
414.898 -0.073981411755085
415.00963 -0.0569524317979813
415.12123 -0.0391393974423409
415.23282 -0.0207635145634413
415.34441 -0.00207599392160773
415.45594 0.0166681539267302
415.5674 0.0352142155170441
415.67888 0.0533207207918167
415.7904 0.0707336440682411
415.90187 0.0871889963746071
416.01325 0.102459393441677
416.12464 0.11634036898613
416.23604 0.128632128238678
416.34739 0.139158979058266
416.4587 0.14778371155262
416.57003 0.154397681355476
416.68141 0.158922806382179
416.79286 0.16130767762661
416.90435 0.161532163619995
417.01585 0.159608766436577
417.12737 0.155576214194298
417.23896 0.149503380060196
417.35065 0.141470551490784
417.46234 0.131598278880119
417.574 0.12002320587635
417.68563 0.106900997459888
417.79731 0.0923846289515495
417.90899 0.0766580179333687
418.02062 0.0599342063069344
418.13218 0.042418647557497
418.24372 0.0243223235011101
418.35522 0.00588467391207814
418.46664 -0.0126562491059303
418.578 -0.0310525503009558
418.68931 -0.0490641742944717
418.80052 -0.0664432868361473
418.91162 -0.0829529613256454
419.02274 -0.0983822047710419
419.13389 -0.112510994076729
419.24497 -0.125135272741318
419.35595 -0.136079102754593
419.467 -0.145207166671753
419.57816 -0.152395069599152
419.68932 -0.157542049884796
419.80044 -0.160581275820732
419.91166 -0.161482870578766
};
\end{axis}

\end{tikzpicture}


==> Python_data_figure/Mes_point_result/ModalPINN_VS_ExpMes_2020_10_29-09_26_24__357/Validation_loss_with_modes.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Number of modes},
xmin=-0.15, xmax=3.15,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={\(\displaystyle 0\),\(\displaystyle 1\),\(\displaystyle 2\),\(\displaystyle 3\)},
y grid style={white!69.0196078431373!black},
ylabel={Normalised Validation Error},
ymin=0.000396112842703244, ymax=1.45214044883202,
ymode=log,
ytick style={color=black},
ytick={1e-05,0.0001,0.001,0.01,0.1,1,10,100},
yticklabels={\(\displaystyle 10^{-5}\),\(\displaystyle 10^{-4}\),\(\displaystyle 10^{-3}\),\(\displaystyle 10^{-2}\),\(\displaystyle 10^{-1}\),\(\displaystyle 10^{0}\),\(\displaystyle 10^{1}\),\(\displaystyle 10^{2}\)}
]
\path [draw=black, semithick, dash pattern=on 5.55pt off 2.4pt]
(axis cs:0,1)
--(axis cs:3,1);

\addplot [semithick, color0, dashed, mark=square*, mark size=3, mark options={solid}]
table {%
0 0.207379162311554
1 0.0130139421671629
2 0.00748647097498178
3 0.00731012364849448
};
\addplot [semithick, color1, dashed, mark=*, mark size=3, mark options={solid}]
table {%
0 0.0176829695701599
1 0.00143955205567181
2 0.000626487308181822
3 0.000575211481191218
};
\addplot [semithick, color2, dashed, mark=triangle*, mark size=3, mark options={solid}]
table {%
0 0.564595460891724
1 0.0321590229868889
2 0.0178603641688824
3 0.0170018896460533
};
\addplot [semithick, color3, dashed, mark=triangle*, mark size=3, mark options={solid,rotate=270}]
table {%
0 0.0398590378463268
1 0.00544324843212962
2 0.00397256063297391
3 0.00435326993465424
};
\end{axis}

\end{tikzpicture}


==> Python_data_figure/Mes_point_result/ModalPINN_VS_ExpMes_Noise_2020_10_16-17_07_01__22-NOTUSED/Forces.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Time \(\displaystyle t\)},
xmin=399.0885955, xmax=420.9032345,
xtick style={color=black},
xtick={395,400,405,410,415,420,425},
xticklabels={\(\displaystyle 395\),\(\displaystyle 400\),\(\displaystyle 405\),\(\displaystyle 410\),\(\displaystyle 415\),\(\displaystyle 420\),\(\displaystyle 425\)},
y grid style={white!69.0196078431373!black},
ylabel={Forces},
ymin=-0.205001482362801, ymax=0.740228789618813,
ytick style={color=black},
ytick={-0.4,-0.2,0,0.2,0.4,0.6,0.8},
yticklabels={\(\displaystyle -0.4\),\(\displaystyle -0.2\),\(\displaystyle 0.0\),\(\displaystyle 0.2\),\(\displaystyle 0.4\),\(\displaystyle 0.6\),\(\displaystyle 0.8\)}
]
\addplot [semithick, color0]
table {%
400.08017 0.66265895
400.19165 0.66180014
400.30305 0.66110401
400.41439 0.66060713
400.52567 0.6603356
400.63684 0.66030324
400.74793 0.66051093
400.85907 0.66094756
400.97021 0.66158977
401.08125 0.66240257
401.19224 0.6633431
401.30333 0.66436308
401.4145 0.66540879
401.52564 0.66642421
401.63678 0.66735637
401.74805 0.66815725
401.85943 0.6687841
401.97082 0.66920296
402.08224 0.66939164
402.19376 0.66933968
402.30533 0.66904914
402.41691 0.66853507
402.52852 0.6678243
402.64015 0.66695439
402.75178 0.66597163
402.86341 0.66492834
402.97502 0.66388043
403.08661 0.66288389
403.1982 0.66199192
403.30973 0.66125251
403.4212 0.66070502
403.53267 0.66037805
403.64419 0.66028896
403.75567 0.66044236
403.86706 0.66082936
403.97844 0.66142915
404.08985 0.66220981
404.20121 0.66312934
404.31252 0.66413878
404.42384 0.66518519
404.53521 0.66621379
404.64665 0.66717047
404.75815 0.66800445
404.86965 0.66867128
404.98116 0.66913569
405.09274 0.66937308
405.20442 0.66937022
405.31612 0.66912668
405.42777 0.66865532
405.53941 0.66798102
405.65108 0.66713912
405.76277 0.66617431
405.8744 0.66513859
405.98597 0.66408754
406.09751 0.66307684
406.20902 0.66216049
406.32045 0.6613877
406.43182 0.66079929
406.54313 0.66042613
406.65435 0.66028768
406.76546 0.66039042
406.87657 0.66072845
406.98773 0.66128389
407.09882 0.66202655
407.20981 0.66291651
407.32085 0.66390784
407.432 0.66494912
407.54316 0.66598468
407.65428 0.66695967
407.76548 0.66782392
407.87683 0.66853216
407.98822 0.66904599
408.09961 0.66933791
408.21109 0.66939236
408.32265 0.66920568
408.43423 0.66878732
408.54582 0.66815908
408.65745 0.66735394
408.76907 0.66641468
408.8807 0.66539128
408.99232 0.66433842
409.10392 0.6633125
409.21551 0.66236824
409.32708 0.66155626
409.43857 0.66092015
409.55003 0.66049333
409.66153 0.6602982
409.77304 0.66034522
409.88447 0.66063135
409.99584 0.66114079
410.10724 0.6618465
410.21863 0.66271064
410.32996 0.66368685
410.44127 0.66472369
410.55261 0.6657669
410.66402 0.66676174
410.7755 0.66765564
410.887 0.66840096
410.9985 0.66895811
411.11004 0.66929772
411.22169 0.66940141
411.33339 0.66926296
411.44506 0.66888945
411.5567 0.66830068
411.66835 0.66752754
411.78004 0.66661077
411.89171 0.66559952
412.0033 0.66454831
412.11484 0.66351306
412.22637 0.66254876
412.33784 0.66170721
412.44923 0.66103326
412.56057 0.66056228
412.67185 0.66031898
412.783 0.66031563
412.89409 0.66055161
413.00524 0.66101439
413.11637 0.66167912
413.22739 0.66250962
413.33839 0.66346235
413.44949 0.66448834
413.56067 0.66553337
413.6718 0.66654149
413.78295 0.66746034
413.89424 0.66824246
414.00562 0.66884592
414.11701 0.6692381
414.22844 0.66939821
414.33997 0.66931726
414.45155 0.66899884
414.56313 0.66845954
414.67474 0.66772749
414.78637 0.66684145
414.898 0.66584857
415.00963 0.66480173
415.12123 0.66375706
415.23282 0.66277033
415.34441 0.66189428
415.45594 0.66117602
415.5674 0.6606537
415.67888 0.6603546
415.7904 0.66029462
415.90187 0.66047678
416.01325 0.66089064
416.12464 0.66151403
416.23604 0.66231375
416.34739 0.66324676
416.4587 0.66426348
416.57003 0.66531066
416.68141 0.66633344
416.79286 0.66727798
416.90435 0.66809409
417.01585 0.66873829
417.12737 0.66917654
417.23896 0.66938555
417.35065 0.66935357
417.46234 0.66908175
417.574 0.6685845
417.68563 0.66788803
417.79731 0.66702885
417.90899 0.66605267
418.02062 0.66501215
418.13218 0.66396302
418.24372 0.66296085
418.35522 0.66205927
418.46664 0.66130663
418.578 0.66074263
418.68931 0.66039686
418.80052 0.66028727
418.91162 0.66041879
419.02274 0.6607841
419.13389 0.66136384
419.24497 0.66212642
419.35595 0.66303107
419.467 0.66403122
419.57816 0.6650748
419.68932 0.66610591
419.80044 0.66707016
419.91166 0.66791798
};
\addplot [semithick, color1, dashed]
table {%
400.08017 0.691233515739441
400.19165 0.690780341625214
400.30305 0.690384149551392
400.41439 0.690029561519623
400.52567 0.689707398414612
400.63684 0.689419627189636
400.74793 0.68917977809906
400.85907 0.689012706279755
400.97021 0.688951730728149
401.08125 0.689032912254333
401.19224 0.689288735389709
401.30333 0.68974232673645
401.4145 0.690399527549744
401.52564 0.691244900226593
401.63678 0.692239463329315
401.74805 0.693321943283081
401.85943 0.694409608840942
401.97082 0.695404052734375
402.08224 0.696203231811523
402.19376 0.696709334850311
402.30533 0.696839272975922
402.41691 0.696535408496857
402.52852 0.69577294588089
402.64015 0.69456672668457
402.75178 0.692970335483551
402.86341 0.691074669361115
402.97502 0.689002394676208
403.08661 0.686896145343781
403.1982 0.684907197952271
403.30973 0.683184444904327
403.4212 0.681856870651245
403.53267 0.681023895740509
403.64419 0.680748581886292
403.75567 0.681050181388855
403.86706 0.681902050971985
403.97844 0.683237016201019
404.08985 0.68495237827301
404.20121 0.686919689178467
404.31252 0.688998460769653
404.42384 0.691045463085175
404.53521 0.692933082580566
404.64665 0.694551467895508
404.75815 0.695821225643158
404.86965 0.696696639060974
404.98116 0.697167813777924
405.09274 0.697258174419403
405.20442 0.697016835212708
405.31612 0.696512401103973
405.42777 0.695824146270752
405.53941 0.695031106472015
405.65108 0.694204390048981
405.76277 0.693402469158173
405.8744 0.692664325237274
405.98597 0.692011654376984
406.09751 0.691448152065277
406.20902 0.690965294837952
406.32045 0.690546989440918
406.43182 0.69017618894577
406.54313 0.689840793609619
406.65435 0.689537405967712
406.76546 0.689274728298187
406.87657 0.689072906970978
406.98773 0.688962399959564
407.09882 0.688978612422943
407.20981 0.689156532287598
407.32085 0.689524114131927
407.432 0.69009530544281
407.54316 0.690863907337189
407.65428 0.691801011562347
407.76548 0.692854940891266
407.87683 0.693951666355133
407.98822 0.694998323917389
408.09961 0.695893228054047
408.21109 0.696535348892212
408.32265 0.69683450460434
408.43423 0.696720123291016
408.54582 0.696153938770294
408.65745 0.695132374763489
408.76907 0.693692743778229
408.8807 0.691911518573761
408.99232 0.689898133277893
409.10392 0.687787771224976
409.21551 0.685730576515198
409.32708 0.683876931667328
409.43857 0.682366967201233
409.55003 0.681313514709473
409.66153 0.68079549074173
409.77304 0.680851757526398
409.88447 0.681475222110748
409.99584 0.682614982128143
410.10724 0.684182584285736
410.21863 0.686060011386871
410.32996 0.688108444213867
410.44127 0.690186023712158
410.55261 0.692156374454498
410.66402 0.693900942802429
410.7755 0.695327043533325
410.887 0.696373224258423
410.9985 0.697015702724457
411.11004 0.697263777256012
411.22169 0.697156250476837
411.33339 0.696754515171051
411.44506 0.696134567260742
411.5567 0.695376813411713
411.66835 0.694556832313538
411.78004 0.693738043308258
411.89171 0.692969024181366
412.0033 0.692278563976288
412.11484 0.691677510738373
412.22637 0.691162049770355
412.33784 0.690718412399292
412.44923 0.690329492092133
412.56057 0.68997985124588
412.67185 0.689662456512451
412.783 0.689380586147308
412.89409 0.689149618148804
413.00524 0.688996016979218
413.11637 0.688953936100006
413.22739 0.689059019088745
413.33839 0.689343273639679
413.44949 0.689826726913452
413.56067 0.690513610839844
413.6718 0.691384136676788
413.78295 0.692396104335785
413.89424 0.693484961986542
414.00562 0.694565117359161
414.11701 0.695537030696869
414.22844 0.696298778057098
414.33997 0.696754217147827
414.45155 0.696822583675385
414.56313 0.696451365947723
414.67474 0.695621728897095
414.78637 0.694353103637695
414.898 0.692705512046814
415.00963 0.690775632858276
415.12123 0.688689351081848
415.23282 0.686590611934662
415.34441 0.684632122516632
415.45594 0.682960331439972
415.5674 0.681700468063354
415.67888 0.680947065353394
415.7904 0.68075704574585
415.90187 0.681142628192902
416.01325 0.682071268558502
416.12464 0.683469653129578
416.23604 0.685231268405914
416.34739 0.687224090099335
416.4587 0.689306557178497
416.57003 0.691338241100311
416.68141 0.693191945552826
416.79286 0.694762825965881
416.90435 0.695976495742798
417.01585 0.696791529655457
417.12737 0.697204530239105
417.23896 0.697241961956024
417.35065 0.696956872940063
417.46234 0.696420073509216
417.574 0.695711314678192
417.68563 0.694909274578094
417.79731 0.694083154201508
417.90899 0.693288087844849
418.02062 0.692561984062195
418.13218 0.691922664642334
418.24372 0.691371858119965
418.35522 0.690899729728699
418.46664 0.69048947095871
418.578 0.69012451171875
418.68931 0.689793825149536
418.80052 0.689495623111725
418.91162 0.689240396022797
419.02274 0.689050137996674
419.13389 0.688956022262573
419.24497 0.688994109630585
419.35595 0.689198911190033
419.467 0.689595818519592
419.57816 0.690196931362152
419.68932 0.690993130207062
419.80044 0.691951394081116
419.91166 0.693016588687897
};
\addplot [semithick, color2, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
400.08017 0.019452365
400.19165 0.00082595482
400.30305 -0.017823055
400.41439 -0.036252194
400.52567 -0.054212695
400.63684 -0.07145315
400.74793 -0.087747648
400.85907 -0.10288897
400.97021 -0.11666154
401.08125 -0.12886365
401.19224 -0.13933821
401.30333 -0.14795541
401.4145 -0.1545944
401.52564 -0.15916143
401.63678 -0.1616036
401.74805 -0.16189495
401.85943 -0.16003304
401.97082 -0.15605006
402.08224 -0.1500052
402.19376 -0.14197773
402.30533 -0.13207828
402.41691 -0.12044238
402.52852 -0.10721965
402.64015 -0.092582119
402.75178 -0.076720103
402.86341 -0.059836271
402.97502 -0.042150431
403.08661 -0.023890474
403.1982 -0.0052916919
403.30973 0.013394412
403.4212 0.031916296
403.53267 0.050037844
403.64419 0.067519465
403.75567 0.0841073
403.86706 0.099566848
403.97844 0.11369648
404.08985 0.12630308
404.20121 0.137206
404.31252 0.14625769
404.42384 0.15334185
404.53521 0.15836743
404.64665 0.16126968
404.75815 0.16201283
404.86965 0.16059349
404.98116 0.15703911
405.09274 0.15140107
405.20442 0.14375595
405.31612 0.13421243
405.42777 0.12290535
405.53941 0.10998327
405.65108 0.095608396
405.76277 0.079966299
405.8744 0.06326761
405.98597 0.045731335
406.09751 0.027576533
406.20902 0.0090389852
406.32045 -0.0096302792
406.43182 -0.028186056
406.54313 -0.046384181
406.65435 -0.063971299
406.76546 -0.080707845
406.87657 -0.096382432
406.98773 -0.11078404
407.09882 -0.12369926
407.20981 -0.13495076
407.32085 -0.14440068
407.432 -0.1519239
407.54316 -0.15741141
407.65428 -0.1607929
407.76548 -0.16203258
407.87683 -0.1611163
407.98822 -0.15806048
408.09961 -0.15291444
408.21109 -0.14574775
408.32265 -0.13665628
408.43423 -0.12576688
408.54582 -0.11322267
408.65745 -0.099184956
408.76907 -0.083837596
408.8807 -0.067377282
408.99232 -0.050016414
409.10392 -0.031980823
409.21551 -0.013501073
409.32708 0.0051782451
409.43857 0.02380233
409.55003 0.042128615
409.66153 0.059922605
409.77304 0.076934714
409.88447 0.092917049
409.99584 0.10765567
410.10724 0.12095599
410.21863 0.13262888
410.32996 0.14251104
410.44127 0.15047359
410.55261 0.15641452
410.66402 0.16025722
410.7755 0.16195275
410.887 0.16148319
410.9985 0.15886317
411.11004 0.15413418
411.22169 0.14736073
411.33339 0.13863711
411.44506 0.12808831
411.5567 0.11585782
411.66835 0.10210092
411.78004 0.086991725
411.89171 0.070730936
412.0033 0.053536419
412.11484 0.035626131
412.22637 0.017226451
412.33784 -0.0014157133
412.44923 -0.020051091
412.56057 -0.038437383
412.67185 -0.056324484
412.783 -0.073462687
412.89409 -0.089629758
413.00524 -0.10461836
413.11637 -0.11821234
413.22739 -0.13021457
413.33839 -0.1404729
413.44949 -0.14885881
413.56067 -0.15525328
413.6718 -0.1595674
413.78295 -0.16175245
413.89424 -0.16178491
414.00562 -0.15966605
414.11701 -0.15543215
414.22844 -0.14914467
414.33997 -0.14088604
414.45155 -0.13077075
414.56313 -0.11893617
414.67474 -0.10553408
414.78637 -0.090739337
414.898 -0.074743672
415.00963 -0.05775169
415.12123 -0.039984874
415.23282 -0.021671532
415.34441 -0.0030487316
415.45594 0.015630664
415.5674 0.034116752
415.67888 0.052174529
415.7904 0.069562324
415.90187 0.086026368
416.01325 0.10133657
416.12464 0.1152936
416.23604 0.12770475
416.34739 0.13839259
416.4587 0.14721378
416.57003 0.15405521
416.68141 0.15882884
416.79286 0.16147326
416.90435 0.1619564
417.01585 0.16027886
417.12737 0.15647128
417.23896 0.15058773
417.35065 0.14270841
417.46234 0.13294577
417.574 0.12143682
417.68563 0.10833146
417.79731 0.093794154
417.90899 0.078013759
418.02062 0.061203035
418.13218 0.043580823
418.24372 0.025367159
418.35522 0.0068005066
418.46664 -0.011867886
418.578 -0.030393829
418.68931 -0.048532063
418.80052 -0.066029138
418.91162 -0.082649052
419.02274 -0.098182302
419.13389 -0.11241644
419.24497 -0.12514037
419.35595 -0.13618249
419.467 -0.14540768
419.57816 -0.15269174
419.68932 -0.15792937
419.80044 -0.16105524
419.91166 -0.16203647
};
\addplot [semithick, color3, dotted]
table {%
400.08017 0.0296425987035036
400.19165 0.0123781785368919
400.30305 -0.00500630075111985
400.41439 -0.0222593285143375
400.52567 -0.0391186326742172
400.63684 -0.0553320907056332
400.74793 -0.0706444010138512
400.85907 -0.0848485305905342
400.97021 -0.0977269262075424
401.08125 -0.109088309109211
401.19224 -0.118797823786736
401.30333 -0.126754060387611
401.4145 -0.132869079709053
401.52564 -0.137094542384148
401.63678 -0.139413356781006
401.74805 -0.139832019805908
401.85943 -0.138370290398598
401.97082 -0.135068699717522
402.08224 -0.129976466298103
402.19376 -0.123152323067188
402.30533 -0.114660926163197
402.41691 -0.104589365422726
402.52852 -0.0930166319012642
402.64015 -0.0800603404641151
402.75178 -0.0658435299992561
402.86341 -0.0505100786685944
402.97502 -0.0342425629496574
403.08661 -0.0172429326921701
403.1982 0.000270266376901418
403.30973 0.0180274341255426
403.4212 0.0357638224959373
403.53267 0.0532131157815456
403.64419 0.0700875073671341
403.75567 0.0861095115542412
403.86706 0.101002350449562
403.97844 0.114549823105335
404.08985 0.126539275050163
404.20121 0.136802896857262
404.31252 0.145214900374413
404.42384 0.151683449745178
404.53521 0.156165778636932
404.64665 0.158642157912254
404.75815 0.159124076366425
404.86965 0.157649248838425
404.98116 0.154277771711349
405.09274 0.149078115820885
405.20442 0.142129957675934
405.31612 0.133524119853973
405.42777 0.123375609517097
405.53941 0.11178132891655
405.65108 0.0988558605313301
405.76277 0.0847463458776474
405.8744 0.069596454501152
405.98597 0.0535852573812008
406.09751 0.0369051769375801
406.20902 0.0197602547705173
406.32045 0.00239608320407569
406.43182 -0.0149448551237583
406.54313 -0.0320022366940975
406.65435 -0.0485223792493343
406.76546 -0.0642448589205742
406.87657 -0.0789439976215363
406.98773 -0.0924146771430969
407.09882 -0.104442812502384
407.20981 -0.114870451390743
407.32085 -0.123585097491741
407.432 -0.13049453496933
407.54316 -0.135528147220612
407.65428 -0.138658583164215
407.76548 -0.139885127544403
407.87683 -0.139220878481865
407.98822 -0.136696770787239
408.09961 -0.132361948490143
408.21109 -0.126266598701477
408.32265 -0.118476085364819
408.43423 -0.109065368771553
408.54582 -0.0981254577636719
408.65745 -0.085742674767971
408.76907 -0.0720424503087997
408.8807 -0.0571671202778816
408.99232 -0.0412761978805065
409.10392 -0.0245595946907997
409.21551 -0.00723838293924928
409.32708 0.0104502532631159
409.43857 0.0282298605889082
409.55003 0.0458289794623852
409.66153 0.0629873126745224
409.77304 0.0794055536389351
409.88447 0.0948108434677124
409.99584 0.108956538140774
410.10724 0.121631309390068
410.21863 0.132652714848518
410.32996 0.141864091157913
410.44127 0.1491689234972
410.55261 0.15450194478035
410.66402 0.157832562923431
410.7755 0.159160852432251
410.887 0.158513650298119
410.9985 0.155941516160965
411.11004 0.151512324810028
411.22169 0.145298317074776
411.33339 0.137385278940201
411.44506 0.127879828214645
411.5567 0.116889253258705
411.66835 0.104519434273243
411.78004 0.0908928140997887
411.89171 0.0761625468730927
412.0033 0.0604993179440498
412.11484 0.0440786629915237
412.22637 0.0271044634282589
412.33784 0.00980549585074186
412.44923 -0.00757245114073157
412.56057 -0.0247855726629496
412.67185 -0.0415708869695663
412.783 -0.0576601177453995
412.89409 -0.0728253722190857
413.00524 -0.0868455395102501
413.11637 -0.0995082035660744
413.22739 -0.110633701086044
413.33839 -0.12008872628212
413.44949 -0.127776294946671
413.56067 -0.133615225553513
413.6718 -0.137558549642563
413.78295 -0.139594882726669
413.89424 -0.139733418822289
414.00562 -0.137996792793274
414.11701 -0.134427294135094
414.22844 -0.129073977470398
414.33997 -0.121999599039555
414.45155 -0.113268785178661
414.56313 -0.102964647114277
414.67474 -0.0911856964230537
414.78637 -0.078031100332737
414.898 -0.0636354461312294
415.00963 -0.0481554083526134
415.12123 -0.0317698903381824
415.23282 -0.0146754560992122
415.34441 0.00288768159225583
415.45594 0.0206604246050119
415.5674 0.0383714735507965
415.67888 0.0557536482810974
415.7904 0.0725232884287834
415.90187 0.0883880108594894
416.01325 0.103095725178719
416.12464 0.116425402462482
416.23604 0.128172561526299
416.34739 0.13816899061203
416.4587 0.146296188235283
416.57003 0.152473896741867
416.68141 0.156659305095673
416.79286 0.158838510513306
416.90435 0.159027770161629
417.01585 0.157269015908241
417.12737 0.153620839118958
417.23896 0.148159146308899
417.35065 0.140958711504936
417.46234 0.132119044661522
417.574 0.121744267642498
417.68563 0.109949037432671
417.79731 0.0968419834971428
417.90899 0.0825609043240547
418.02062 0.0672749578952789
418.13218 0.051155086606741
418.24372 0.0343878716230392
418.35522 0.0171979479491711
418.46664 -0.000180015049409121
418.578 -0.0174927767366171
418.68931 -0.0344882160425186
418.80052 -0.0509040839970112
418.91162 -0.0664904117584229
419.02274 -0.0810267254710197
419.13389 -0.0942928940057755
419.24497 -0.10609420388937
419.35595 -0.116274312138557
419.467 -0.124725200235844
419.57816 -0.131358280777931
419.68932 -0.13611264526844
419.80044 -0.13896045088768
419.91166 -0.139905422925949
};
\end{axis}

\end{tikzpicture}


==> Python_data_figure/Noise_dependency/figure_Noise_dependency.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.19140625,0.515625,0.53125}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Noise Level \(\displaystyle \sigma\)},
xmin=8e-05, xmax=0.12,
xmode=log,
xtick style={color=black},
xtick={1e-07,1e-05,0.001,0.1,10,1000},
xticklabels={\(\displaystyle 10^{-7}\),\(\displaystyle 10^{-5}\),\(\displaystyle 10^{-3}\),\(\displaystyle 10^{-1}\),\(\displaystyle 10^{1}\),\(\displaystyle 10^{3}\)},
y grid style={white!69.0196078431373!black},
ylabel={Validation Loss},
ymin=0.00122097816, ymax=0.053872776,
ymode=log,
ytick style={color=black},
ytick={0.0001,0.001,0.01,0.1,1},
yticklabels={\(\displaystyle 10^{-4}\),\(\displaystyle 10^{-3}\),\(\displaystyle 10^{-2}\),\(\displaystyle 10^{-1}\),\(\displaystyle 10^{0}\)}
]
\path [draw=color0, fill=color0, opacity=0.5]
(axis cs:0.0001,0.00179432092)
--(axis cs:0.0001,0.0288906974)
--(axis cs:0.001,0.0117954606)
--(axis cs:0.002,0.0318523677)
--(axis cs:0.005,0.0309098928)
--(axis cs:0.01,0.0211077123)
--(axis cs:0.02,0.01485440415)
--(axis cs:0.05,0.029546492)
--(axis cs:0.1,0.0197554132)
--(axis cs:0.1,0.00249362198)
--(axis cs:0.1,0.00249362198)
--(axis cs:0.05,0.00217277025)
--(axis cs:0.02,0.00173823928)
--(axis cs:0.01,0.00162604609)
--(axis cs:0.005,0.00167503317)
--(axis cs:0.002,0.00165811752)
--(axis cs:0.001,0.00173598064)
--(axis cs:0.0001,0.00179432092)
--cycle;

\addplot [only marks, mark=+, draw=black, fill=black, colormap/viridis]
table{%
x                      y
0.001 0.008660569
0.001 0.0018421422
0.001 0.0020232282
0.001 0.0027906275
0.01 0.001775617
0.01 0.021058764
0.001 0.020975225
0.01 0.012391648
0.01 0.010459118
0.01 0.008627019
0.1 0.028827665
0.1 0.0037311274
0.1 0.0047155293
0.1 0.0024790787
0.1 0.002833598
0.005 0.012252242
0.005 0.0056138313
0.002 0.0017393164
0.002 0.0016654041
0.002 0.0019369287
0.005 0.04489398
0.002 0.026624229
0.002 0.014563084
0.005 0.0024057
0.005 0.02306655
0.02 0.0122710075
0.02 0.038104974
0.02 0.0029205242
0.05 0.0021755458
0.02 0.0019390828
0.02 0.0017415918
0.05 0.028646594
0.0001 0.0034542999
0.05 0.01654495
0.05 0.010980628
0.001 0.0022731654
0.0001 0.001970097
0.001 0.003634121
0.0001 0.002026505
0.05 0.0022930466
0.0001 0.0018235882
0.0001 0.0017260306
0.0001 0.001625618
0.0001 0.015959777
0.002 0.005329346
0.0001 0.038331553
0.0001 0.030560441
0.002 0.0019331095
0.001 0.010793594
0.002 0.0018074231
0.001 0.003122324
0.002 0.036963213
0.005 0.0016470358
0.01 0.001573499
0.01 0.0017333366
0.002 0.0015925383
0.005 0.0016762717
0.005 0.0018448826
0.005 0.0020898955
0.01 0.0020205178
0.005 0.029365674
0.01 0.021548247
0.01 0.0015885574
0.02 0.04449328
0.02 0.002490145
0.02 0.001725217
0.02 0.0016712783
0.02 0.002634939
0.05 0.0027887186
0.05 0.0023311388
0.05 0.040286645
0.05 0.0022780183
0.05 0.014245883
0.1 0.0027692225
0.1 0.019625539
0.1 0.015559679
0.1 0.0023740546
0.1 0.020924281
0.01 0.0055547007
0.01 0.004349732
0.01 0.0018162619
0.01 0.0017186796
0.01 0.0021504574
0.1 0.002604348
0.1 0.017540526
0.1 0.003726256
0.1 0.01342753
0.1 0.00880955
0.1 0.0041593276
0.1 0.003405613
0.1 0.0028312774
0.1 0.0024952379
0.1 0.017407387
0.05 0.034898423
0.05 0.0022774462
0.05 0.005863114
0.05 0.0024421848
0.05 0.0025833522
0.05 0.017451424
0.05 0.0021320807
0.05 0.028951833
0.05 0.0071912482
0.05 0.0021477903
0.02 0.0022694485
0.02 0.007407465
0.02 0.0058862376
0.02 0.0017801215
0.02 0.0017396862
0.02 0.01008157
0.02 0.009395516
0.02 0.0018172308
0.02 0.002133251
0.02 0.0019345491
0.01 0.023050796
0.01 0.008242319
0.01 0.009791701
0.005 0.00219163
0.01 0.0024580392
0.01 0.0016302115
0.001 0.0072963014
0.005 0.007266371
0.002 0.0039271927
0.005 0.0059848316
0.002 0.005975843
0.002 0.0039073033
0.005 0.003812363
0.002 0.0025383953
0.005 0.0017343094
0.001 0.0053647626
0.001 0.0017588809
0.005 0.0016638864
0.0001 0.0022726269
0.005 0.0188903
0.001 0.002087364
0.002 0.0015878378
0.002 0.0022193433
0.001 0.0015262227
0.002 0.0021967364
0.002 0.0019396063
0.001 0.0020684048
0.005 0.0017549298
0.0001 0.0020631868
0.0001 0.0022556053
0.001 0.0018377726
0.0001 0.0019021237
0.0001 0.002201475
0.001 0.0018274329
0.002 0.040189978
0.005 0.029191319
0.005 0.044807862
0.001 0.0016443796
0.002 0.031284496
0.0001 0.028175093
0.0001 0.009555669
0.001 0.015802927
0.0001 0.015399131
0.0001 0.0021434932
};
\addplot [only marks, mark=o, draw=red, colormap/viridis]
table{%
x                      y
0.1 0.00901234137
0.05 0.011425503225
0.01 0.007176961105
0.005 0.012107693255
0.02 0.007721855765
0.0001 0.00908035075555556
0.002 0.00949606621
0.001 0.00512260235789474
};

\nextgroupplot[
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Noise Level \(\displaystyle \sigma\)},
xmin=8e-05, xmax=0.12,
xmode=log,
xtick style={color=black},
xtick={1e-07,1e-05,0.001,0.1,10,1000},
xticklabels={\(\displaystyle 10^{-7}\),\(\displaystyle 10^{-5}\),\(\displaystyle 10^{-3}\),\(\displaystyle 10^{-1}\),\(\displaystyle 10^{1}\),\(\displaystyle 10^{3}\)},
y grid style={white!69.0196078431373!black},
ylabel={Equations Loss},
ymin=0.000278531456, ymax=4.7064144,
ymode=log,
ytick style={color=black},
ytick={1e-06,0.0001,0.01,1,100,10000},
yticklabels={\(\displaystyle 10^{-6}\),\(\displaystyle 10^{-4}\),\(\displaystyle 10^{-2}\),\(\displaystyle 10^{0}\),\(\displaystyle 10^{2}\),\(\displaystyle 10^{4}\)}
]
\path [draw=color0, fill=color0, opacity=0.5]
(axis cs:0.0001,0.000480410449)
--(axis cs:0.0001,0.01142621291)
--(axis cs:0.001,0.0100291303)
--(axis cs:0.002,0.171270636)
--(axis cs:0.005,0.0173443793)
--(axis cs:0.01,0.0432654775)
--(axis cs:0.02,0.0183767196)
--(axis cs:0.05,0.0140323796)
--(axis cs:0.1,0.00688785824)
--(axis cs:0.1,0.00059399913)
--(axis cs:0.1,0.00059399913)
--(axis cs:0.05,0.000412949833)
--(axis cs:0.02,0.000392994872)
--(axis cs:0.01,0.000543093947)
--(axis cs:0.005,0.000493247627)
--(axis cs:0.002,0.000529545763)
--(axis cs:0.001,0.000535064128)
--(axis cs:0.0001,0.000480410449)
--cycle;

\addplot [only marks, mark=+, draw=black, fill=black, colormap/viridis]
table{%
x                      y
0.001 0.031215528
0.001 0.00053858536
0.001 0.0017295592
0.001 0.002447654
0.01 0.0008233254
0.01 0.0049891
0.001 0.0037527608
0.01 0.001677599
0.01 0.0012391127
0.01 0.0026399544
0.1 0.008666984
0.1 0.0011785895
0.1 0.00058156275
0.1 0.0006924813
0.1 0.0014144192
0.005 0.074065275
0.005 0.0015705848
0.002 0.0004425168
0.002 0.00083410565
0.002 0.0012607285
0.005 0.009428392
0.002 0.01637891
0.002 0.0034187923
0.005 0.0053120386
0.005 0.0051103826
0.02 0.0027206326
0.02 0.019282386
0.02 0.0005423872
0.05 0.0006017681
0.02 0.00040089907
0.02 0.00057002064
0.05 0.008158272
0.0001 0.00069246243
0.05 0.0203147
0.05 0.0031991191
0.001 0.0114150075
0.0001 0.0009998897
0.001 0.0047236355
0.0001 0.0040692785
0.05 0.0005115744
0.0001 0.00043273123
0.0001 0.0014779256
0.0001 0.0005008444
0.0001 0.020259092
0.002 0.1477113
0.0001 0.0076406933
0.0001 0.07654351
0.002 0.0017970914
0.001 0.0034306038
0.002 0.00053872215
0.001 0.0015243541
0.002 3.922012
0.005 0.0012576544
0.01 0.00054964103
0.01 0.00045106313
0.002 0.0004480993
0.005 0.00039275878
0.005 0.0004999324
0.005 0.000750552
0.01 0.0013405068
0.005 0.028534766
0.01 0.005895278
0.01 0.041611202
0.02 0.01827609
0.02 0.0010276635
0.02 0.00040160445
0.02 0.00039564408
0.02 0.008803944
0.05 0.00042087576
0.05 0.82879674
0.05 0.008287304
0.05 0.0010960569
0.05 0.0020561914
0.1 0.0005909619
0.1 0.018265303
0.1 0.0051732934
0.1 0.0005943366
0.1 0.0043890225
0.01 0.06562312
0.01 0.0010088823
0.01 0.00072845834
0.01 0.0006146678
0.01 0.0012344993
0.1 0.0008000099
0.1 0.006446563
0.1 0.0005970497
0.1 0.0032507218
0.1 0.0066901776
0.1 0.00077304564
0.1 0.0006413275
0.1 0.00093229656
0.1 0.0011406016
0.1 0.0045957607
0.05 0.009231693
0.05 0.0004127479
0.05 0.0015666626
0.05 0.00041297227
0.05 0.00034816432
0.05 0.009073162
0.05 0.00090188376
0.05 0.013334344
0.05 0.0018589172
0.05 0.00042453845
0.02 0.00042144247
0.02 0.030676914
0.02 0.0009808374
0.02 0.00041795793
0.02 0.0005397116
0.02 0.0022982683
0.02 0.00390687
0.02 0.000369152
0.02 0.00035090497
0.02 0.0008983309
0.01 0.058153957
0.01 0.0009664084
0.01 0.0119315265
0.005 0.0014262622
0.01 0.0015832073
0.01 0.0004841702
0.001 0.009682661
0.005 0.0035612707
0.002 0.38330466
0.005 0.0013416592
0.002 0.09590953
0.002 0.0025056803
0.005 0.016101003
0.002 0.0034947356
0.005 0.00062606257
0.001 0.0039624674
0.001 0.0006679185
0.005 0.00043308467
0.0001 0.002070623
0.005 0.0043135546
0.001 0.0013641424
0.002 0.00053859537
0.002 0.0018592823
0.001 0.00044642045
0.002 0.0034140414
0.002 0.0017730326
0.001 0.004898156
0.005 0.0006366283
0.0001 0.000615597
0.0001 0.0020412293
0.001 0.0013149213
0.0001 0.0003707455
0.0001 0.0019480188
0.001 0.0005209792
0.002 0.009683699
0.005 0.009846367
0.005 0.011483892
0.001 0.0010000895
0.002 0.030297706
0.0001 0.0072073387
0.0001 0.004216682
0.001 0.0032900858
0.0001 0.0030788907
0.0001 0.0005812752
};
\addplot [only marks, mark=o, draw=red, colormap/viridis]
table{%
x                      y
0.1 0.0033707254075
0.05 0.045550384358
0.01 0.01017728398
0.005 0.008834606041
0.02 0.0046640830555
0.0001 0.00748593485333333
0.002 0.2313811614335
0.001 0.00462765946368421
};

\nextgroupplot[
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Noise Level \(\displaystyle \sigma\)},
xmin=8e-05, xmax=0.12,
xmode=log,
xtick style={color=black},
xtick={1e-07,1e-05,0.001,0.1,10,1000},
xticklabels={\(\displaystyle 10^{-7}\),\(\displaystyle 10^{-5}\),\(\displaystyle 10^{-3}\),\(\displaystyle 10^{-1}\),\(\displaystyle 10^{1}\),\(\displaystyle 10^{3}\)},
y grid style={white!69.0196078431373!black},
ylabel={Loss Pitot},
ymin=7.9297504e-05, ymax=0.024462372,
ymode=log,
ytick style={color=black},
ytick={1e-07,1e-05,0.001,0.1,10},
yticklabels={\(\displaystyle 10^{-7}\),\(\displaystyle 10^{-5}\),\(\displaystyle 10^{-3}\),\(\displaystyle 10^{-1}\),\(\displaystyle 10^{1}\)}
]
\path [draw=color0, fill=color0, opacity=0.5]
(axis cs:0.0001,9.99269045e-05)
--(axis cs:0.0001,0.000334137029)
--(axis cs:0.001,0.000222056888)
--(axis cs:0.002,0.000360183146)
--(axis cs:0.005,0.000681040195)
--(axis cs:0.01,0.000551441624)
--(axis cs:0.02,0.00107748557)
--(axis cs:0.05,0.00545325103)
--(axis cs:0.1,0.0201969237)
--(axis cs:0.1,0.0196014562)
--(axis cs:0.1,0.0196014562)
--(axis cs:0.05,0.00498961475)
--(axis cs:0.02,0.000882719112)
--(axis cs:0.01,0.000295152885)
--(axis cs:0.005,0.000147171414)
--(axis cs:0.002,0.0001095155384)
--(axis cs:0.001,0.00010242383)
--(axis cs:0.0001,9.99269045e-05)
--cycle;

\addplot [only marks, mark=+, draw=black, fill=black, colormap/viridis]
table{%
x                      y
0.001 0.0001586225
0.001 0.000103373364
0.001 0.00010333708
0.001 0.00010404588
0.01 0.0003021395
0.01 0.0005507409
0.001 0.00031150633
0.01 0.00042419892
0.01 0.0004071462
0.01 0.000419208
0.1 0.02038531
0.1 0.020040028
0.1 0.019716507
0.1 0.019853655
0.1 0.020008285
0.005 0.00018653616
0.005 0.00022920148
0.002 0.0001101228
0.002 0.00011005558
0.002 0.000108353444
0.005 0.0007169695
0.002 0.0002915948
0.002 0.00022744983
0.005 0.00014718511
0.005 0.00037929253
0.02 0.0010471551
0.02 0.001556588
0.02 0.0008846158
0.05 0.0050215134
0.02 0.0009011839
0.02 0.00088361884
0.05 0.005592542
0.0001 0.00012299938
0.05 0.0051895804
0.05 0.005064384
0.001 0.000111530426
0.0001 9.978289e-05
0.001 0.00011043694
0.0001 0.00010060248
0.05 0.0049706427
0.0001 0.0001019514
0.0001 9.912188e-05
0.0001 0.00010110331
0.0001 0.00028614045
0.002 0.00012041131
0.0001 0.0006765406
0.0001 0.0002748873
0.002 0.000112664864
0.001 0.00020931325
0.002 0.00010658141
0.001 0.000108816086
0.002 0.00033557904
0.005 0.0001504225
0.01 0.00029319664
0.01 0.00029567492
0.002 0.00010964466
0.005 0.00014907404
0.005 0.00014738298
0.005 0.00014697612
0.01 0.0003006824
0.005 0.0005246465
0.01 0.00055774814
0.01 0.00029523575
0.02 0.0013504598
0.02 0.00087462156
0.02 0.0008990457
0.02 0.0008660103
0.02 0.0008925597
0.05 0.004989964
0.05 0.00503185
0.05 0.0054492867
0.05 0.0050152643
0.05 0.005177369
0.1 0.019846587
0.1 0.020176215
0.1 0.020383302
0.1 0.02002646
0.1 0.019965576
0.01 0.0003119158
0.01 0.0003062415
0.01 0.00029914748
0.01 0.00029989367
0.01 0.00029886
0.1 0.019774118
0.1 0.02015336
0.1 0.019869316
0.1 0.019603312
0.1 0.020070296
0.1 0.019635057
0.1 0.019584754
0.1 0.019758679
0.1 0.019514924
0.1 0.020006847
0.05 0.00548893
0.05 0.005009012
0.05 0.005027362
0.05 0.0049864715
0.05 0.005077103
0.05 0.005154544
0.05 0.0050853454
0.05 0.005310514
0.05 0.005011934
0.05 0.0050106463
0.02 0.00089102704
0.02 0.00093654386
0.02 0.00089436764
0.02 0.00089661276
0.02 0.0009071887
0.02 0.0009838396
0.02 0.0010154567
0.02 0.00088826224
0.02 0.0009021841
0.02 0.0008879932
0.01 0.0005632525
0.01 0.00042219853
0.01 0.0003652737
0.005 0.00015461797
0.01 0.0002944071
0.01 0.0002998017
0.001 0.0001547299
0.005 0.000217365
0.002 0.00011577769
0.005 0.00016238193
0.002 0.00013308812
0.002 0.00011414497
0.005 0.00015502101
0.002 0.0001135266
0.005 0.00015294092
0.001 0.00012042604
0.001 0.000106966705
0.005 0.00014844682
0.0001 0.000102232996
0.005 0.0005434428
0.001 0.000102846185
0.002 0.00011008375
0.002 0.00011133427
0.001 0.00010517665
0.002 0.00011067197
0.002 0.00011109763
0.001 0.00010408412
0.005 0.00014704815
0.0001 0.000104923216
0.0001 0.00010341133
0.001 0.00010255547
0.0001 0.00010100766
0.0001 0.000103293416
0.001 0.00010189727
0.002 0.00059928244
0.005 0.00067704805
0.005 0.0007174326
0.001 0.000100032565
0.002 0.0005816201
0.0001 0.0003730532
0.0001 0.00019570759
0.001 0.00027303144
0.0001 0.00031745867
0.0001 9.9988625e-05
};
\addplot [only marks, mark=o, draw=red, colormap/viridis]
table{%
x                      y
0.1 0.0199186294
0.05 0.005133212935
0.01 0.0003653481675
0.005 0.0002926716085
0.02 0.000967966727
0.0001 0.000186900355166667
0.002 0.0001866542639
0.001 0.000136459379
};
\addplot [semithick, black, dashed]
table {%
0.1 0.02
0.008 0.000128
};
\draw (axis cs:0.015,0.00015) node[
  scale=0.9,
  anchor=base west,
  text=black,
  rotate=0.0
]{2:1};

\nextgroupplot[
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Noise Level \(\displaystyle \sigma\)},
xmin=8e-05, xmax=0.12,
xmode=log,
xtick style={color=black},
xtick={1e-07,1e-05,0.001,0.1,10,1000},
xticklabels={\(\displaystyle 10^{-7}\),\(\displaystyle 10^{-5}\),\(\displaystyle 10^{-3}\),\(\displaystyle 10^{-1}\),\(\displaystyle 10^{1}\),\(\displaystyle 10^{3}\)},
y grid style={white!69.0196078431373!black},
ylabel={Loss Cylinder},
ymin=5.00529312e-07, ymax=0.0123687612,
ymode=log,
ytick style={color=black},
ytick={1e-09,1e-07,1e-05,0.001,0.1,10},
yticklabels={\(\displaystyle 10^{-9}\),\(\displaystyle 10^{-7}\),\(\displaystyle 10^{-5}\),\(\displaystyle 10^{-3}\),\(\displaystyle 10^{-1}\),\(\displaystyle 10^{1}\)}
]
\path [draw=color0, fill=color0, opacity=0.5]
(axis cs:0.0001,1.013869368e-06)
--(axis cs:0.0001,0.00030111736)
--(axis cs:0.001,0.000125894548)
--(axis cs:0.002,0.000274344305)
--(axis cs:0.005,0.000440115197)
--(axis cs:0.01,0.000290606228)
--(axis cs:0.02,0.000519073764000001)
--(axis cs:0.05,0.00279337019)
--(axis cs:0.1,0.0100618336)
--(axis cs:0.1,0.0096241312)
--(axis cs:0.1,0.0096241312)
--(axis cs:0.05,0.0024100234)
--(axis cs:0.02,0.000389415269)
--(axis cs:0.01,9.94104814e-05)
--(axis cs:0.005,2.55226996e-05)
--(axis cs:0.002,5.14442396e-06)
--(axis cs:0.001,2.47633768e-06)
--(axis cs:0.0001,1.013869368e-06)
--cycle;

\addplot [only marks, mark=+, draw=black, fill=black, colormap/viridis]
table{%
x                      y
0.001 1.1783618e-05
0.001 2.6516393e-06
0.001 2.6671053e-06
0.001 2.4963385e-06
0.01 9.7919845e-05
0.01 0.00027602262
0.001 0.00016379745
0.01 0.00015054167
0.01 0.00011944067
0.01 0.00011644172
0.1 0.009974154
0.1 0.009964204
0.1 0.009666484
0.1 0.00950707
0.1 0.009830659
0.005 3.8331407e-05
0.005 3.8773112e-05
0.002 5.4069487e-06
0.002 4.9061396e-06
0.002 5.8304017e-06
0.005 0.00043038017
0.002 0.00023006539
0.002 0.0001559973
0.005 2.4808565e-05
0.005 0.00033816838
0.02 0.00047816674
0.02 0.0009181308
0.02 0.00040210265
0.05 0.0024438666
0.02 0.0003955555
0.02 0.00038997844
0.05 0.0027897076
0.0001 7.002562e-06
0.05 0.002580856
0.05 0.0025043613
0.001 3.1870545e-06
0.0001 9.0519336e-07
0.001 4.029682e-06
0.0001 2.1930196e-06
0.05 0.0024186224
0.0001 5.451328e-06
0.0001 1.4441728e-06
0.0001 1.168469e-06
0.0001 0.00022403443
0.002 9.673003e-06
0.0001 0.00048097753
0.0001 0.00016506718
0.002 7.185846e-06
0.001 0.00012052144
0.002 5.2383525e-06
0.001 5.701989e-06
0.002 0.0010542355
0.005 2.5997351e-05
0.01 0.000102126134
0.01 9.949284e-05
0.002 5.1709e-06
0.005 2.714476e-05
0.005 2.5765103e-05
0.005 2.5573754e-05
0.01 9.8669254e-05
0.005 0.0004278384
0.01 0.00047806697
0.01 0.000100687685
0.02 0.0008834586
0.02 0.0004241619
0.02 0.00040184974
0.02 0.000403697
0.02 0.0004327736
0.05 0.00239371
0.05 0.0025152906
0.05 0.0030247683
0.05 0.002403556
0.05 0.0025187256
0.1 0.009946177
0.1 0.009987119
0.1 0.009819829
0.1 0.00992696
0.1 0.010071514
0.01 0.000102926984
0.01 0.00010254775
0.01 0.00010121501
0.01 0.00010137868
0.01 0.00010026984
0.1 0.009766801
0.1 0.010060758
0.1 0.009494193
0.1 0.009993763
0.1 0.010021346
0.1 0.009885001
0.1 0.010307301
0.1 0.009849242
0.1 0.009637138
0.1 0.009950108
0.05 0.0028263335
0.05 0.002410742
0.05 0.0025522127
0.05 0.0025333108
0.05 0.0024430603
0.05 0.0025254665
0.05 0.0024333263
0.05 0.002620432
0.05 0.0025345085
0.05 0.0024875563
0.02 0.00040029152
0.02 0.00044238113
0.02 0.00040031725
0.02 0.00038576213
0.02 0.00039161244
0.02 0.00047858656
0.02 0.00045305042
0.02 0.00038885573
0.02 0.00038947744
0.02 0.0004309833
0.01 0.0004218587
0.01 0.000115245195
0.01 0.00016069027
0.005 2.6576881e-05
0.01 0.000102084516
0.01 0.0001012076
0.001 1.9394076e-05
0.005 4.085686e-05
0.002 8.350249e-06
0.005 3.0749547e-05
0.002 1.2968548e-05
0.002 7.5092294e-06
0.005 2.935262e-05
0.002 6.6135744e-06
0.005 2.583456e-05
0.001 1.0859813e-05
0.001 3.6570439e-06
0.005 2.5119001e-05
0.0001 1.7904999e-06
0.005 0.00018894026
0.001 3.4151992e-06
0.002 6.0015577e-06
0.002 5.563871e-06
0.001 2.3963344e-06
0.002 5.6786057e-06
0.002 4.739396e-06
0.001 2.7712672e-06
0.005 2.5567555e-05
0.0001 1.4566228e-06
0.0001 2.3761909e-06
0.001 2.2488666e-06
0.0001 1.0604448e-06
0.0001 1.9618494e-06
0.001 2.886137e-06
0.002 0.00025932177
0.005 0.00075944705
0.005 0.00052773044
0.001 2.9043204e-06
0.002 0.00040954712
0.0001 0.000568899
0.0001 4.2265954e-05
0.001 0.00014738698
0.0001 8.806186e-05
0.0001 6.2566164e-07
};
\addplot [only marks, mark=o, draw=red, colormap/viridis]
table{%
x                      y
0.1 0.00988299105
0.05 0.002548020665
0.01 0.00015244169765
0.005 0.0001541477888
0.02 0.0004645596445
0.0001 8.87078871222222e-05
0.002 0.000110500185135
0.001 2.70924397e-05
};
\addplot [semithick, black, dashed]
table {%
0.1 0.01
0.001 1e-06
};
\draw (axis cs:0.005,2.7e-06) node[
  scale=0.9,
  anchor=base west,
  text=black,
  rotate=0.0
]{2:1};
\end{groupplot}

\end{tikzpicture}

